MEEL: Multi-Modal Event Evolution Learning

Multi-modal Event Reasoning (MMER) endeavors to endow machines with the ability to comprehend intricate event relations across diverse data modalities. MMER is fundamental and underlies a wide broad of applications. Despite extensive instruction fine-tuning, current multi-modal large language models still fall short in such ability. The disparity stems from that existing models are insufficient to capture underlying principles governing event evolution in various scenarios. In this paper, we introduce Multi-Modal Event Evolution Learning (MEEL) to enable the model to grasp the event evolution mechanism, yielding advanced MMER ability. Specifically, we commence with the design of event diversification to gather seed events from a rich spectrum of scenarios. Subsequently, we employ ChatGPT to generate evolving graphs for these seed events. We propose an instruction encapsulation process that formulates the evolving graphs into instruction-tuning data, aligning the comprehension of event reasoning to humans. Finally, we observe that models trained in this way are still struggling to fully comprehend event evolution. In such a case, we propose the guiding discrimination strategy, in which models are trained to discriminate the improper evolution direction. We collect and curate a benchmark M-EV2 for MMER. Extensive experiments on M-EV2 validate the effectiveness of our approach, showcasing competitive performance in open-source multi-modal LLMs.

==> custom.tex <==
# event definition
@article{tao2023eveval,
  title={EvEval: A Comprehensive Evaluation of Event Semantics for Large Language Models},
  author={Tao, Zhengwei and Jin, Zhi and Bai, Xiaoying and Zhao, Haiyan and Feng, Yanlin and Li, Jia and Hu, Wenpeng},
  journal={arXiv preprint arXiv:2305.15268},
  year={2023}
}


@article{vendler1957verbs,
  title={Verbs and times},
  author={Vendler, Zeno},
  journal={The philosophical review},
  pages={143--160},
  year={1957},
  publisher={JSTOR}
}

@inproceedings{doddington2004automatic,
  title={The automatic content extraction (ace) program-tasks, data, and evaluation.},
  author={Mitchell, Alexis},
  year={2005},
}


# understanding 
@article{pedinotti2021did,
  title={Did the cat drink the coffee? Challenging transformers with generalized event knowledge},
  author={Pedinotti, Paolo and Rambelli, Giulia and Chersoni, Emmanuele and Santus, Enrico and Lenci, Alessandro and Blache, Philippe},
  journal={arXiv preprint arXiv:2107.10922},
  year={2021}
}

# reasoning
@inproceedings{han2021ester,
  title={ESTER: A machine reading comprehension dataset for reasoning about event semantic relations},
  author={Han, Rujun and Hsu, I-Hung and Sun, Jiao and Baylon, Julia and Ning, Qiang and Roth, Dan and Peng, Nanyun},
  booktitle={Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing},
  pages={7543--7559},
  year={2021}
}

@inproceedings{yang2020temporal,
  title={A temporal semantic search system for traditional Chinese medicine based on temporal knowledge graphs},
  author={Yang, Chengbiao and Li, Weizhuo and Zhang, Xiaoping and Zhang, Runshun and Qi, Guilin},
  booktitle={Semantic Technology: 9th Joint International Conference, JIST 2019, Hangzhou, China, November 25--27, 2019, Revised Selected Papers 9},
  pages={13--20},
  year={2020},
  organization={Springer}
}

@inproceedings{souza2020event,
  title={Event-QA: A dataset for event-centric question answering over knowledge graphs},
  author={Souza Costa, Tarc{\'\i}sio and Gottschalk, Simon and Demidova, Elena},
  booktitle={Proceedings of the 29th ACM international conference on information \& knowledge management},
  pages={3157--3164},
  year={2020}
}

@article{gao2023chatgpt,
  title={Is ChatGPT a Good Causal Reasoner? A Comprehensive Evaluation},
  author={Gao, Jinglong and Ding, Xiao and Qin, Bing and Liu, Ting},
  journal={arXiv preprint arXiv:2305.07375},
  year={2023}
}

@article{du2022care,
  title={e-CARE: a new dataset for exploring explainable causal reasoning},
  author={Du, Li and Ding, Xiao and Xiong, Kai and Liu, Ting and Qin, Bing},
  journal={arXiv preprint arXiv:2205.05849},
  year={2022}
}

@article{xu2024survey,
  title={A survey on knowledge distillation of large language models},
  author={Xu, Xiaohan and Li, Ming and Tao, Chongyang and Shen, Tao and Cheng, Reynold and Li, Jinyang and Xu, Can and Tao, Dacheng and Zhou, Tianyi},
  journal={arXiv preprint arXiv:2402.13116},
  year={2024}
}


@article{zhou2019going,
  title={" Going on a vacation" takes longer than" Going for a walk": A Study of Temporal Commonsense Understanding},
  author={Zhou, Ben and Khashabi, Daniel and Ning, Qiang and Roth, Dan},
  journal={arXiv preprint arXiv:1909.03065},
  year={2019}
}

@article{sap2019socialiqa,
  title={Socialiqa: Commonsense reasoning about social interactions},
  author={Sap, Maarten and Rashkin, Hannah and Chen, Derek and LeBras, Ronan and Choi, Yejin},
  journal={arXiv preprint arXiv:1904.09728},
  year={2019}
}

@inproceedings{mostafazadeh2016corpus,
  title={A corpus and cloze evaluation for deeper understanding of commonsense stories},
  author={Mostafazadeh, Nasrin and Chambers, Nathanael and He, Xiaodong and Parikh, Devi and Batra, Dhruv and Vanderwende, Lucy and Kohli, Pushmeet and Allen, James},
  booktitle={Proceedings of the 2016 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  pages={839--849},
  year={2016}
}

@article{poria2021recognizing,
  title={Recognizing emotion cause in conversations},
  author={Poria, Soujanya and Majumder, Navonil and Hazarika, Devamanyu and Ghosal, Deepanway and Bhardwaj, Rishabh and Jian, Samson Yu Bai and Hong, Pengfei and Ghosh, Romila and Roy, Abhinaba and Chhaya, Niyati and others},
  journal={Cognitive Computation},
  volume={13},
  pages={1317--1332},
  year={2021},
  publisher={Springer}
}


@article{yang2022towards,
  title={Towards Fine-grained Causal Reasoning and QA},
  author={Yang, Linyi and Wang, Zhen and Wu, Yuxiang and Yang, Jie and Zhang, Yue},
  journal={arXiv preprint arXiv:2204.07408},
  year={2022}
}

@article{qin2019counterfactual,
  title={Counterfactual story reasoning and generation},
  author={Qin, Lianhui and Bosselut, Antoine and Holtzman, Ari and Bhagavatula, Chandra and Clark, Elizabeth and Choi, Yejin},
  journal={arXiv preprint arXiv:1909.04076},
  year={2019}
}

@article{qin2020back,
  title={Back to the future: Unsupervised backprop-based decoding for counterfactual and abductive commonsense reasoning},
  author={Qin, Lianhui and Shwartz, Vered and West, Peter and Bhagavatula, Chandra and Hwang, Jena and Bras, Ronan Le and Bosselut, Antoine and Choi, Yejin},
  journal={arXiv preprint arXiv:2010.05906},
  year={2020}
}

@inproceedings{tao2023unievent,
  title={UniEvent: Unified Generative Model with Multi-Dimensional Prefix for Zero-Shot Event-Relational Reasoning},
  author={Tao, Zhengwei and Jin, Zhi and Zhao, Haiyan and Dou, Chengfeng and Zhao, Yongqiang and Shen, Tao and Tao, Chongyang},
  booktitle={Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={7088--7102},
  year={2023}
}

@inproceedings{tao2023seag,
  title={SEAG: Structure-Aware Event Causality Generation},
  author={Tao, Zhengwei and Jin, Zhi and Bai, Xiaoying and Zhao, Haiyan and Dou, Chengfeng and Zhao, Yongqiang and Wang, Fang and Tao, Chongyang},
  booktitle={Findings of the Association for Computational Linguistics: ACL 2023},
  pages={4631--4644},
  year={2023}
}

% prediction
@article{zhao2021event,
  title={Event prediction in the big data era: A systematic survey},
  author={Zhao, Liang},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={5},
  pages={1--37},
  year={2021},
  publisher={ACM New York, NY, USA}
}


@inproceedings{guan2019story,
  title={Story ending generation with incremental encoding and commonsense knowledge},
  author={Guan, Jian and Wang, Yansen and Huang, Minlie},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={6473--6480},
  year={2019}
}

# llm
@article{chung2022scaling,
  title={Scaling instruction-finetuned language models},
  author={Chung, Hyung Won and Hou, Le and Longpre, Shayne and Zoph, Barret and Tay, Yi and Fedus, William and Li, Eric and Wang, Xuezhi and Dehghani, Mostafa and Brahma, Siddhartha and others},
  journal={arXiv preprint arXiv:2210.11416},
  year={2022}
}

@article{touvron2023llama,
  title={Llama: Open and efficient foundation language models},
  author={Touvron, Hugo and Lavril, Thibaut and Izacard, Gautier and Martinet, Xavier and Lachaux, Marie-Anne and Lacroix, Timoth{\'e}e and Rozi{\`e}re, Baptiste and Goyal, Naman and Hambro, Eric and Azhar, Faisal and others},
  journal={arXiv preprint arXiv:2302.13971},
  year={2023}
}

@misc{alpaca,
  author = {Rohan Taori and Ishaan Gulrajani and Tianyi Zhang and Yann Dubois and Xuechen Li and Carlos Guestrin and Percy Liang and Tatsunori B. Hashimoto },
  title = {Stanford Alpaca: An Instruction-following LLaMA model},
  year = {2023},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/tatsu-lab/stanford_alpaca}},
}

@article{muennighoff2022crosslingual,
  title={Crosslingual generalization through multitask finetuning},
  author={Muennighoff, Niklas and Wang, Thomas and Sutawika, Lintang and Roberts, Adam and Biderman, Stella and Scao, Teven Le and Bari, M Saiful and Shen, Sheng and Yong, Zheng-Xin and Schoelkopf, Hailey and others},
  journal={arXiv preprint arXiv:2211.01786},
  year={2022}
}

@misc{vicuna2023,
    title = {Vicuna: An Open-Source Chatbot Impressing GPT-4 with 90\%* ChatGPT Quality},
    url = {https://lmsys.org/blog/2023-03-30-vicuna/},
    author = {Chiang, Wei-Lin and Li, Zhuohan and Lin, Zi and Sheng, Ying and Wu, Zhanghao and Zhang, Hao and Zheng, Lianmin and Zhuang, Siyuan and Zhuang, Yonghao and Gonzalez, Joseph E. and Stoica, Ion and Xing, Eric P.},
    month = {March},
    year = {2023}
}

@article{xu2023wizardlm,
  title={Wizardlm: Empowering large language models to follow complex instructions},
  author={Xu, Can and Sun, Qingfeng and Zheng, Kai and Geng, Xiubo and Zhao, Pu and Feng, Jiazhan and Tao, Chongyang and Jiang, Daxin},
  journal={arXiv preprint arXiv:2304.12244},
  year={2023}
}

@online{DatabricksBlog2023DollyV2,
    title = {Free Dolly: Introducing the World's First Truly Open Instruction-Tuned LLM},
    author = {Conover, Mike and Hayes, Matt and Mathur, Ankit and Xie, Jianwei and Wan, Jun and Shah, Sam and Ghodsi, Ali and Wendell, Patrick and Zaharia, Matei and Xin, Reynold},
    year = {2023},
    
}

@article{openai2023gpt,
  title={GPT-4 technical report},
  author={OpenAI, R},
  journal={arXiv},
  pages={2303--08774},
  year={2023}
}

@article{ouyang2022training,
  title={Training language models to follow instructions with human feedback},
  author={Ouyang, Long and Wu, Jeffrey and Jiang, Xu and Almeida, Diogo and Wainwright, Carroll and Mishkin, Pamela and Zhang, Chong and Agarwal, Sandhini and Slama, Katarina and Ray, Alex and others},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={27730--27744},
  year={2022}
}


# event 
@inproceedings{zhang2020aser,
  title={ASER: A large-scale eventuality knowledge graph},
  author={Zhang, Hongming and Liu, Xin and Pan, Haojie and Song, Yangqiu and Leung, Cane Wing-Ki},
  booktitle={Proceedings of the web conference 2020},
  pages={201--211},
  year={2020}
}

@inproceedings{zhou2022eventbert,
  title={Eventbert: A pre-trained model for event correlation reasoning},
  author={Zhou, Yucheng and Geng, Xiubo and Shen, Tao and Long, Guodong and Jiang, Daxin},
  booktitle={Proceedings of the ACM Web Conference 2022},
  pages={850--859},
  year={2022}
}

@inproceedings{zhou2022claret,
  title={ClarET: Pre-training a Correlation-Aware Context-To-Event Transformer for Event-Centric Generation and Classification},
  author={Zhou, Yucheng and Shen, Tao and Geng, Xiubo and Long, Guodong and Jiang, Daxin},
  booktitle={Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={2559--2575},
  year={2022}
}

@inproceedings{zhu2015aligning,
  title={Aligning books and movies: Towards story-like visual explanations by watching movies and reading books},
  author={Zhu, Yukun and Kiros, Ryan and Zemel, Rich and Salakhutdinov, Ruslan and Urtasun, Raquel and Torralba, Antonio and Fidler, Sanja},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={19--27},
  year={2015}
}

@inproceedings{prasad2008penn,
  title={The Penn Discourse TreeBank 2.0.},
  author={Prasad, Rashmi and Dinesh, Nikhil and Lee, Alan and Miltsakaki, Eleni and Robaldo, Livio and Joshi, Aravind K and Webber, Bonnie L},
  booktitle={LREC},
  year={2008}
}

# metrics
@inproceedings{papineni2002bleu,
  title={Bleu: a method for automatic evaluation of machine translation},
  author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
  booktitle={Proceedings of the 40th annual meeting of the Association for Computational Linguistics},
  pages={311--318},
  year={2002}
}

@inproceedings{lin2004rouge,
  title={Rouge: A package for automatic evaluation of summaries},
  author={Lin, Chin-Yew},
  booktitle={Text summarization branches out},
  pages={74--81},
  year={2004}
}

@article{zhang2019bertscore,
  title={Bertscore: Evaluating text generation with bert},
  author={Zhang, Tianyi and Kishore, Varsha and Wu, Felix and Weinberger, Kilian Q and Artzi, Yoav},
  journal={arXiv preprint arXiv:1904.09675},
  year={2019}
}

@article{zhang2023huatuogpt,
  title={HuatuoGPT, towards Taming Language Model to Be a Doctor},
  author={Zhang, Hongbo and Chen, Junying and Jiang, Feng and Yu, Fei and Chen, Zhihong and Li, Jianquan and Chen, Guiming and Wu, Xiangbo and Zhang, Zhiyi and Xiao, Qingying and others},
  journal={arXiv preprint arXiv:2305.15075},
  year={2023}
}

@article{fan2023grammargpt,
  title={GrammarGPT: Exploring Open-Source LLMs for Native Chinese Grammatical Error Correction with Supervised Fine-Tuning},
  author={Fan, Yaxin and Jiang, Feng and Li, Peifeng and Li, Haizhou},
  journal={arXiv preprint arXiv:2307.13923},
  year={2023}
}

@article{cui2023chatlaw,
  title={ChatLaw: Open-Source Legal Large Language Model with Integrated External Knowledge Bases},
  author={Cui, Jiaxi and Li, Zongjian and Yan, Yang and Chen, Bohua and Yuan, Li},
  journal={arXiv preprint arXiv:2306.16092},
  year={2023}
}

@article{deepke-llm,
  author = {Zhang, Ningyu and Zhang, Jintian and Wang, Xiaohan and Gui, Honghao and Jiang, Yinuo and Chen, Xiang and Mao, Shengyu and Qiao, Shuofei and Bi, Zhen and Chen, Jing and Liang, Xiaozhuan and Ou, Yixin and Fang, Ruinan and Xi, Zekun and Xu, Xin and Tao, Liankuan and Li, Lei and Wang, Peng and Li, Zhoubo and Zheng, Guozhou and Chen, Huajun},
  title = {DeepKE-LLM: A Large Language Model Based Knowledge Extraction Toolkit},
  year = {2023},
  publisher = {GitHub}
}


@article{yang2023fingpt,
  title={FinGPT: Open-Source Financial Large Language Models},
  author={Yang, Hongyang and Liu, Xiao-Yang and Wang, Christina Dan},
  journal={arXiv preprint arXiv:2306.06031},
  year={2023}
}

@article{tang2023toolalpaca,
  title={ToolAlpaca: Generalized Tool Learning for Language Models with 3000 Simulated Cases},
  author={Tang, Qiaoyu and Deng, Ziliang and Lin, Hongyu and Han, Xianpei and Liang, Qiao and Sun, Le},
  journal={arXiv preprint arXiv:2306.05301},
  year={2023}
}

@article{yu2020cocolm,
  title={CoCoLM: Complex commonsense enhanced language model with discourse relations},
  author={Yu, Changlong and Zhang, Hongming and Song, Yangqiu and Ng, Wilfred},
  journal={arXiv preprint arXiv:2012.15643},
  year={2020}
}

@article{liu2023agentbench,
  title={Agentbench: Evaluating llms as agents},
  author={Liu, Xiao and Yu, Hao and Zhang, Hanchen and Xu, Yifan and Lei, Xuanyu and Lai, Hanyu and Gu, Yu and Ding, Hangliang and Men, Kaiwen and Yang, Kejuan and others},
  journal={arXiv preprint arXiv:2308.03688},
  year={2023}
}

@inproceedings{ning2018multi,
  title={A Multi-Axis Annotation Scheme for Event Temporal Relations},
  author={Ning, Qiang and Wu, Hao and Roth, Dan},
  booktitle={Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={1318--1328},
  year={2018}
}

@inproceedings{caselli2017event,
  title={The event storyline corpus: A new benchmark for causal and temporal relation extraction},
  author={Caselli, Tommaso and Vossen, Piek},
  booktitle={Proceedings of the Events and Stories in the News Workshop},
  pages={77--86},
  year={2017}
}

@article{wang2022self,
  title={Self-instruct: Aligning language model with self generated instructions},
  author={Wang, Yizhong and Kordi, Yeganeh and Mishra, Swaroop and Liu, Alisa and Smith, Noah A and Khashabi, Daniel and Hajishirzi, Hannaneh},
  journal={arXiv preprint arXiv:2212.10560},
  year={2022}
}

@article{rafailov2023direct,
  title={Direct preference optimization: Your language model is secretly a reward model},
  author={Rafailov, Rafael and Sharma, Archit and Mitchell, Eric and Ermon, Stefano and Manning, Christopher D and Finn, Chelsea},
  journal={arXiv preprint arXiv:2305.18290},
  year={2023}
}

@article{bai2023qwen,
  title={Qwen technical report},
  author={Bai, Jinze and Bai, Shuai and Chu, Yunfei and Cui, Zeyu and Dang, Kai and Deng, Xiaodong and Fan, Yang and Ge, Wenbin and Han, Yu and Huang, Fei and others},
  journal={arXiv preprint arXiv:2309.16609},
  year={2023}
}

@article{jiang2023mistral,
  title={Mistral 7B},
  author={Jiang, Albert Q and Sablayrolles, Alexandre and Mensch, Arthur and Bamford, Chris and Chaplot, Devendra Singh and Casas, Diego de las and Bressand, Florian and Lengyel, Gianna and Lample, Guillaume and Saulnier, Lucile and others},
  journal={arXiv preprint arXiv:2310.06825},
  year={2023}
}

@inproceedings{wang2022ecckg,
  title={ECCKG: An Eventuality-Centric Commonsense Knowledge Graph},
  author={Wang, Ya and Cao, Cungen and Chen, Zhiwen and Wang, Shi},
  booktitle={International Conference on Knowledge Science, Engineering and Management},
  pages={568--584},
  year={2022},
  organization={Springer}
}

@article{hu2021lora,
  title={Lora: Low-rank adaptation of large language models},
  author={Hu, Edward J and Shen, Yelong and Wallis, Phillip and Allen-Zhu, Zeyuan and Li, Yuanzhi and Wang, Shean and Wang, Lu and Chen, Weizhu},
  journal={arXiv preprint arXiv:2106.09685},
  year={2021}
}


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


